Front-running Attack in Sharded Blockchains and Fair Cross-shard Consensus

Sharding is a prominent technique for scaling blockchains. By dividing the network into smaller components known as shards, a sharded blockchain can process transactions in parallel without introducing inconsistencies through the coordination of intra-shard and cross-shard consensus protocols. However, we observe a critical security issue with sharded systems: transaction ordering manipulations can occur when coordinating intra-shard and cross-shard consensus protocols, leaving the system vulnerable to attack. Specifically, we identify a novel security issue known as finalization fairness, which can be exploited through a front-running attack. This attack allows an attacker to manipulate the execution order of transactions, even if the victim's transaction has already been processed and added to the blockchain by a fair intra-shard consensus. To address the issue, we offer Haechi, a novel cross-shard protocol that is immune to front-running attacks. Haechi introduces an ordering phase between transaction processing and execution, ensuring that the execution order of transactions is the same as the processing order and achieving finalization fairness. To accommodate different consensus speeds among shards, Haechi incorporates a finalization fairness algorithm to achieve a globally fair order with minimal performance loss. By providing a global order, Haechi ensures strong consistency among shards, enabling better parallelism in handling conflicting transactions across shards. These features make Haechi a promising solution for supporting popular smart contracts in the real world. To evaluate Haechi's performance, we implemented the protocol using Tendermint and conducted extensive experiments on a geo-distributed AWS environment. Our results demonstrate that Haechi achieves finalization fairness with little performance sacrifice compared to existing cross-shard consensus protocols.

==> acknowledgement.tex <==
\section*{Acknowledgement}\label{sec-ack}
The authors would like to thank all the anonymous reviewers for their valuable comments to improve this paper. The work is partially supported by the National Key Research and Development Plan (2021YFB2700302), the National Natural Science Foundation of China (62172453), the National Natural Science Foundation of Guangdong province (2022A1515010154), the Major Key Project of PCL (PCL2021A06), the Pearl River Talent Recruitment Program (No. 2019QN01X130), and the National Science Foundation
(NSF) under grant CNS1846316.

==> appendics/apdx-proof.tex <==
\section{Security Proof}\label{sec-security-proof-detail}
In this section, we will give detailed proof for the finalization fairness, safety, and liveness of Haechi under the assumption in \cref{section3-trust-model}.

\subsection{Proof of Finalization Fairness}\label{appendix-finalization-fairness-proof}
Recall from the definition in \cref{section3-fairness-definition}, finalization fairness indicates that if two transactions are involved in calling the same contract, then their execution orders (i.e., finalization orders) in all contracts they are jointly involved in are the same as their processing order. In Haechi, transaction execution and commitment follow the global order established in the ordering phase. Therefore, we can prove that Haechi provides finalization fairness by showing that the ordering of transactions in the ordering phase follows the processing order strictly. Note that the beacon chain works in ordering cycles, in each of which the beacon chain picks received CrossLinks selectively and orders OTXs in them.

\begin{lemma}\label{lemma-finalization-fairness-inflight}
    In Haechi, the block timestamp of any in-flight CrossLink is larger than all block timestamps of CrossLinks that are ordered in the current ordering cycling.
\end{lemma}
\begin{myproof}{}
    We prove this lemma by comparing: (i) in-flight CrossLinks with the received CrossLinks from the same shard; (ii) in-flight CrossLinks with the received CrossLinks from different shards.

    \noindent (i) First, in our finalization fairness algorithm (Algorithm \ref{alg-order}), the beacon chain starts ordering in the current ordering cycle once it receives at least one CrossLink with a consecutive block height from each shard. On the one hand, \emph{at least one} ensures that the beacon chain will not miss CrossLinks from any shard in the current ordering cycle. On the other hand, the \emph{consecutive block height} ensures that all CrossLinks corresponding to blocks with smaller block heights have been received in the current ordering cycle or ordered in the previous ordering cycles. Therefore, for every shard, all its in-flight CrossLinks have a higher block timestamp than its CrossLinks received by the beacon chain in the current ordering cycle.

    \noindent (ii) Second, assume $S_i.CL_{last}$ is the last received CrossLink and $\{S_i.CL_{flight}\}$ is a set of all in-flight CrossLinks from $S_i$. In the current ordering cycle, the largest timestamp (i.e., $endTS$ in the algorithm) that is allowed to be ordered is the minimum block timestamp of the last received CrossLinks among all shards. Without loss of generality, we assume $S_1.CL_{last}$ has the minimum block timestamp in the current ordering cycle, and there are $m$ shard chains. Then, we have:
    \begin{equation}
    \label{eq-last-block}
        S_1.CL_{last}.blockTS \leq S_i.CL_{last}.blockTS,
    \end{equation}
    where $1 < i \leq m$. Moreover, according to Proof (i) we can know all in-flight CrossLinks of a shard have a higher block timestamp than the shard's last CrossLink that is received by the beacon chain. Thus, for all shards $S_i$ ($1 \leq i \leq m$) and any CrossLink $cl \in \{S_i.CL_{flight}\}$, we have:
    \begin{equation}
    \label{eq-flight-block}
        S_i.CL_{last}.blockTS < cl.blockTS.
    \end{equation}
    
    Finally, from Equations (\ref{eq-last-block}) and (\ref{eq-flight-block}), we can finally show:
    \begin{equation}
        S_1.CL_{last}.blockTS \leq cl.blockTS,
    \end{equation}
    where $\forall cl \in \{S_i.CL_{flight}\}$ and $1 \leq i \leq m$. In other words, the block timestamp of any in-flight CrossLink is larger than all block timestamps of CrossLinks that are ordered in the current ordering cycling.
\end{myproof}

\begin{lemma}\label{lemma-finalization-fairness-order}
    For any two received transactions $OTX^1$ and $OTX^2$, piggybacked by CrossLinks $CL_1$ and $CL_2$ respectively, if (i) $CL_1.blockTS < CL_2.blockTS$, or (ii) $CL_1 = CL_2$ and $f_{idx}(OTX^1) < f_{idx}(OTX^2)$, then Haechi must order $OTX^1$ before $OTX^2$ in the ordering phase.
\end{lemma}
\begin{myproof}{}
    Note that $f_{idx}(\cdot)$ in Lemma \ref{lemma-finalization-fairness-order} is a function returning the indexes of transactions in a block, same as that of Definition \ref{definition-processing-order}. Moreover, conditions (i) and (ii) in Lemma \ref{lemma-finalization-fairness-order} are actually consistent with the ordering rules we defined in the finalization ordering algorithm (cf. \cref{section:haechi details-ordering phase} step (c)). We now prove Lemma \ref{lemma-finalization-fairness-order} by analyzing all possible byzantine behaviors performed by a malicious leader in the beacon chain.
    
    On the one hand, since the ordering phase is driven by an instance of intra-shard consensus, and $f_{idx}(\cdot)$ and block timestamps are publicly verifiable, a new block created by a malicious leader will not be accepted by other consensus nodes if it contains a transaction order violating the ordering rules, e.g., a transaction with a larger index is ordered before another transaction in the same CrossLink. On the other hand, the malicious leader may deliberately drop some CrossLinks it received, leading that transactions in these dropped CrossLinks are not ordered in the appropriate ordering cycles, thus violating the ordering rules. However, consensus nodes can detect such an omission behavior by checking if the selected CrossLinks in the new block have consecutive block heights for each shard and if the last CrossLinks of all shards are considered in the new block. Overall, any byzantine behaviors violating the ordering rules can be detected and prevented. Since the ordering rules are satisfied all the time, Lemma \ref{lemma-finalization-fairness-order} is correct and the proof is done.
\end{myproof}

With Lemmas \ref{lemma-finalization-fairness-inflight} and \ref{lemma-finalization-fairness-order}, we now prove Theorem \ref{theorem-finalization-fairness}:

\begin{myproof}{ of Theorem \ref{theorem-finalization-fairness}}
    Lemmas \ref{lemma-finalization-fairness-inflight} and \ref{lemma-finalization-fairness-order} guarantee all in-flight and received CrossLinks must be ordered based on the ordering rules. Since the block timestamp and transaction indexes in the ordering rules indicate the processing order, the beacon chain will keep this order for the following execution and commit phases. Therefore, Haechi ensures that the processing order is consistent with the execution order, i.e., ensuring the finalization fairness.
\end{myproof}

\subsection{Proof of Safety}
We show that Haechi guarantees the sharded system safety property by respectively showing Haechi satisfies the two conditions in Definition \ref{def-system-safety}.
\begin{lemma}\label{lemma-intra-shard-consistency}
    For every two honest nodes $N_i^1$ and $N_i^2$ with local ledgers $\mathfrak{L_i}^1$ and $\mathfrak{L_i}^2$ in any shard $S_i$, Haechi guarantees: for all block height $h$ ($0\leq h \leq min\{f_{len}(\mathfrak{L_i}^1), f_{len}(\mathfrak{L_i}^2)\}$), $\mathfrak{L_i}^1[h] = \mathfrak{L_i}^2[h]$, where $f_{len}(\cdot)$ computes the current block height of a chain.
\end{lemma}

\begin{myproof}{}
    Since each shard runs a BFT consensus for maintaining its own ledger and each shard is controlled by the honest nodes (see the trust assumptions in \cref{section3-trust-model}), the shard satisfies the intra-shard safety according to the safety properties of BFT-based protocol. Furthermore, Haechi does not violate the security of the intra-shard consensus. Therefore, $N_i^1$ and $N_i^2$, which participate in the same shard, have a consistent ledger in Haechi. 
\end{myproof}

\begin{lemma}\label{lemma-inter-shard-consistency}
    If an OTX involves the modification of several data managed by multiple shards, then all the relevant shards either commit their local modification or abort it.
\end{lemma}
\begin{myproof}{}
    Recall from \cref{section: architecture} that the transaction sender's shard in Haechi is responsible for coordinating the cross-shard consensus of an OTX. Once nodes of the sender's shard receive messages from all shards relevant to the transaction, the sender's shard runs a BFT-based intra-shard consensus to make a decision based on the received messages. Since the sender's shard is controlled by the honest nodes, such a consensus can be completed securely and generate one commitment decision for the transaction. Since there is no equivocation, all relevant shards will receive a consistent commitment decision on whether to commit or abort their local modification for the transaction. Moreover, the finalization fairness provided by Haechi (cf. Theorem \ref{theorem-finalization-fairness}) ensures the transaction is eventually committed or aborted.
\end{myproof}

With Lemmas \ref{lemma-intra-shard-consistency} and \ref{lemma-inter-shard-consistency}, we now prove Theorem \ref{theorem-system-safety}:

\begin{myproof}{ of Theorem \ref{theorem-system-safety}}
    If the two nodes belong to the same shard, by Lemma \ref{lemma-intra-shard-consistency}, they can keep a consistent ledger via the intra-shard consensus protocol. In other words, these two nodes have the same commitment sequence and operation (i.e., commit or abort) for all transactions recorded in their shard chain. On the other hand, if the two nodes belong to different shards, by Lemma \ref{lemma-inter-shard-consistency}, they can take consistent action to every OSC transaction via Haechi, i.e., either all commit or all abort transactions. Furthermore, since Haechi ensures finalization fairness where the processing order is the same as the commitment order, these two nodes will have the same commitment sequence for all OSC transactions they involve. Together, these observations imply the desired result, i.e., Haechi satisfies the sharded system safety property. 
\end{myproof}

\subsection{Proof of Liveness}
We now give brief proof to show that Haechi satisfies the liveness property of a sharded system.

\begin{myproof}{ of Theorem \ref{theorem-system-liveness}}
    Based on the type of transaction, there are two conditions for handling a transaction $TX$:

    \noindent (i) $TX$ is a non-OTX. In this case, $TX$ will be handled via the original consensus protocol of the sharded system. Specifically, if $TX$ is an intra-shard transaction of a shard, then the shard is responsible for handling it via the intra-shard consensus protocol. If $TX$ is a cross-shard transaction, then all relevant shards collaboratively handle it via the 2P cross-shard consensus protocol. But in either case, the user can receive a response from the sharded system, which is ensured by the underlying protocol of the sharded system.

    \noindent (ii) $TX$ is an OTX. As messages between two honest parties cannot be dropped, the beacon chain eventually receives a CrossLink containing $TX$. Besides, the finalization fairness provided by Haechi guarantees that there is no CrossLink being dropped (otherwise, it violates the finalization fairness since transactions in the dropped CrossLinks cannot be ordered fairly). Since an honest shard is responsive according to the intra-shard liveness provided by the intra-shard BFT protocol. Haechi ensures that any OTX is handled and can get a response eventually.
    
    According to the above analysis, we can conclude that Haechi satisfies the sharded system liveness property.
\end{myproof}




==> package.tex <==
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{paralist}
\ifieee
\usepackage[cmex10]{amsmath}
\usepackage{amssymb,amsfonts,amsthm}
\else
\usepackage{amsmath,amsfonts,amsthm}
\fi
\ifieee
\interdisplaylinepenalty=2500
\fi
%\usepackage[algoruled,linesnumbered,vlined,noend]{algorithm2e}
\usepackage{algorithm}% http://ctan.org/pkg/algorithms
\usepackage{algpseudocode}
\usepackage{graphicx}
\usepackage{booktabs}
% Table packages
\usepackage{tabularx}
\usepackage{varwidth}
\usepackage{array}
\usepackage{adjustbox}
\usepackage{subcaption}
\usepackage{mwe}
\usepackage{textcomp}
\usepackage{comment}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{mathtools}
\usepackage{threeparttable}
% \usepackage[dvipsnames]{xcolor}
\usepackage{xspace}
% \usepackage[hidelinks]{hyperref}
% \hypersetup{
% 	colorlinks=true,
% 	linkcolor=blue,
% 	urlcolor=blue,
% 	citecolor=blue,
% }

%\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
	%T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}

%\usepackage{tablefootnote}
\usepackage{thmtools}
\usepackage[english]{babel}
\usepackage{float}
% For the nice cross mark in the related works table
\usepackage{pifont}
\usepackage{capt-of}
\iffull
  \usepackage[hyphens]{url}
\else
  \usepackage{url}
\fi
\usepackage[inline]{enumitem}
% This hack is for long URLs
\def\UrlBreaks{\do\/\do-}
\iffull
\usepackage[breaklinks]{hyperref}
\fi
\hypersetup{breaklinks=true}
\iffull
  \usepackage{balance}
\fi
% Beautiful Tables
\usepackage{array}
% Proper handling of double column floats
% \usepackage{stfloats}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{definition}{Definition}[section]

\usepackage{tikz}
\usetikzlibrary{backgrounds}
\usetikzlibrary{shapes,shapes.geometric,shapes.symbols,arrows,positioning}
\usetikzlibrary{plotmarks}
\tikzstyle{block} = [rectangle, draw, text width=1cm, 
                     text centered, rounded corners, 
                     minimum height=1cm, node distance=1cm]
\tikzstyle{process} = [circle, draw, text width=1cm, 
                     text centered, rounded corners, 
                     node distance=1cm]
\tikzstyle{line} = [draw, -latex']
\tikzstyle{bubble} = [cloud, draw, text width=1cm, 
                     text centered, rounded corners, 
                     minimum height=1cm, node distance=2cm]

\iffull
\usepackage{changepage}
\fi

==> security-analysis.tex <==
\section{Security Analysis}\label{sec-security-proof-sketch}
In this section, we provide a proof sketch of the finalization fairness, safety, and liveness of Haechi. The detailed proofs are deferred in Appendix \ref{sec-security-proof-detail}.

\subsection{Proof Sketch of Finalization Fairness}
\begin{theorem}\label{theorem-finalization-fairness}
    Haechi provides the finalization fairness for a sharded system.
\end{theorem}
\begin{proofSketch}
    In the ordering phase of Haechi, two transactions are ordered based on the transaction index if they are in the same shard block where they are processed, or based on the block timestamp if they are in different shard blocks. Both the transaction index and block timestamp can indicate the processing order. Namely, the smaller the transaction index or timestamp is, the earlier a transaction is processed. After the ordering phase, these ordered transactions are forwarded to relevant shards for execution (i.e., the execution phase of Haechi). Therefore, the finalization order of transactions is consistent with their processing order. According to the definition in \ref{def-finalization-fariness}, Haechi guarantees the finalization fairness.
\end{proofSketch}

\subsection{Proof Sketch of Safety and Liveness}
A sharded system is a multi-chain ledger where each shard maintains a blockchain via an intra-shard BFT consensus protocol. Each shard can therefore be considered a BFT State Machine Replication (BFT-SMR). However, since cross-shard transactions can modify the data of more than one shard simultaneously, it is not enough to use the original safety and liveness property (cf. intra-shard safety and liveness in \cref{section3-trust-model}) of BFT-SMR to completely describe the security of a sharded system. Therefore, we first define safety and liveness for a sharded system before the proof:
\begin{definition}[Sharded System Safety]\label{def-system-safety}
    A sharded system is said to satisfy the safety property if: (i) any two honest nodes of the same shard maintain the same prefix ledger; (ii) any two honest nodes from two different shards have the same commitment sequence and same operation (commit or abort) for all cross-shard transactions involving the two shards.
\end{definition}

\begin{definition}[Sharded System Liveness]\label{def-system-liveness}
    Every transaction received by at least one honest node will be eventually handled by relevant shards and get a response from the sharded system.
\end{definition}

\begin{theorem}\label{theorem-system-safety}
    Haechi guarantees the sharded system safety.
\end{theorem}

\begin{proofSketch}
    Haechi is a cross-shard consensus protocol built on the intra-shard consensus. For two honest nodes in the same shard, the intra-shard safety of the BFT intra-shard consensus guarantees the first condition of the definition of sharded system safety. When handling cross-shard transactions, the participants (i.e., each shard) of Haechi are all honest without equivocation in cross-shard communications. Moreover, the finalization fairness provided by Haechi ensures the consistency of commitment order. Therefore, Haechi guarantees the second condition of Definition \ref{def-system-safety}. Eventually, Haechi guarantees the sharded system safety.
\end{proofSketch}

\begin{theorem}\label{theorem-system-liveness}
    Haechi guarantees the sharded system's liveness.
\end{theorem}

\begin{proofSketch}
    First, the intra-shard liveness provided by the BFT intra-shard consensus ensures that all transactions will be processed. Since each block of a shard is corresponding to a CrossLink, transactions after being processed are forwarded to the beacon chain with the CrossLink. Then, as messages between two honest parties cannot be dropped, %under the assumption of a partially synchronous network, 
 the beacon chain eventually receives the CrossLink.   %within an unknown delay $\Delta$.

 Since Haechi provides the finalization fairness, the beacon chain will not ignore ordering any CrossLink (otherwise, transactions of an unordered CrossLink are not ordered fairly, resulting in contradiction). Therefore, the transaction can be eventually executed and committed, and its client can get execution the result from  relevant shards.
\end{proofSketch}
